Can We Talk Models Into Seeing the World Differently?

Unlike traditional vision-only models, vision language models (VLMs) offer an intuitive way to access visual content through language prompting by combining a large language model (LLM) with a vision encoder. However, both the LLM and the vision encoder come with their own set of biases, cue preferences, and shortcuts, which have been rigorously studied in uni-modal models. A timely question is how such (potentially misaligned) biases and cue preferences behave under multi-modal fusion in VLMs. As a first step towards a better understanding, we investigate a particularly well-studied vision-only bias - the texture vs. shape bias and the dominance of local over global information. As expected, we find that VLMs inherit this bias to some extent from their vision encoders. Surprisingly, the multi-modality alone proves to have important effects on the model behavior, i.e., the joint training and the language querying change the way visual cues are processed. While this direct impact of language-informed training on a model's visual perception is intriguing, it raises further questions on our ability to actively steer a model's output so that its prediction is based on particular visual cues of the user's choice. Interestingly, VLMs have an inherent tendency to recognize objects based on shape information, which is different from what a plain vision encoder would do. Further active steering towards shape-based classifications through language prompts is however limited. In contrast, active VLM steering towards texture-based decisions through simple natural language prompts is often more successful. URL: https://github.com/paulgavrikov/vlm_shapebias

==> drafts.tex <==









==> skelleton.tex <==
IMPORTANT:
- remove notes on CNN CLIPs -> this is out of scope
- Fill out checklist and make sure it matches openreview answers.

- We previously had vision models and we had language models.
- It's unclear how those modalities interact in vision-language models.
- We ask whether we can *talk* models into *seeing* the world differently.
- That's a broad question, we specifically focus on whether we can take a well-established purely *visual* bias (shape/texture bias) and steer the model output more towards one or the other based on language alone.
- We find that this is indeed the case, providing evidence that 
- This provides evidence that when it comes to visual biases, the output of multimodal models can be influenced through language alone.

Title: Can we talk models into seeing the world differently?
Sections 1-3: Intro, related work, method
Section 4: Shape bias: How do vision-language models see the world?
Section 5: Why do vision-language see the world as they do? [perhaps referencing Kurt Koffka's "Why do things look the way they do?"]
Section 6: Can we talk vision-language models into seeing the world differently?
Section 7: Discussion



Storyline: 
- general impact: alignment of learning models with human perception. Shape bias is a good proxy to investigate alignment: It is well studied misalignment between humans and most models, it can be measured and is intuitive to understand  
- Recognition models have perception biases and steering such biases typically requires retraining
- LLM-based models allow to flexibly steer the task, does this also apply to biases?
- if so, we could easily align model output without retraining
- case study on a bias that achieved much attention: the texture/shape bias

# sec 2: Related Work
- add general alignment lit

# Sec. 3: Method
3.1. Measuring shape bias in recognition tasks
3.2. Recognition tasks in VLMs
- Image Captioning
- VQA Classification
-- Measuring confidence

# Sec. 4: Are VLMs Biased towards Texture or Shape?
4.1 Main results 
=> Establish main overview
Experiment: measure shape bias results of the entire model zoo in both tasks
Results:
- VLMs more shape-biased than ImageNet models, or CLIP
- task does not seem to influence the shape bias significantly
- most VLMs rather similar in terms of shape bias
- models that fail to follow VQA tend to be highly texture biased -> spurious?
- GPT4 outlier with almost 50\% shape bias
- More random facts: RLHF + scale


# Sec. 5. Where does the shape bias come from?
=> Understand how the final prediction is formed

5.1 Role of the vision encoder
=> is the bias purely driven by the vision encoder?
2 Experiments
Experiment 1: Ablate the shape bias of the encoders (CLIP) separately to the entire models 
Results:
- VLMs deviate by -9.5 to +7.4\% in shape bias, accuracy of VLM drops (unsurprisingly) => language seems to impact the bias

Experiment 2: Measure the error consistency on cue-conflict between VLMs, encoders, other models, humans
- VLMs have a high error consistency of up to 79.8\% to the encoders => still over 20\% room for "own" decisions
- Generally high correlation with CLIP predictions (except CNN-based CLIP)
- Choice of LLM does not seem to impact error consistency => seems like data matters most (currently not discussed)
(- other results: high similarity to humans)

=> why is the encoder shape biased? (ViT > CNN is well known, but CLIP > ViT not so much)
Hypothesis: The joint training of text/vision increases shape bias
Negative Result: ResNet-50 CNN does even increase in texture bias (20.8 vs 22.2)

5.2 Processing by the LLM
=> how does the LLM process the vision representation
Experiment: measure the confidence of LLaVA in VQA (this may or may not generalize to other models)
Results:
- VQA predictions are highly confident (almost 100\%) in either shape or texture answers. Almost no cases where confidence is balanced. 2nd most likely token does usually not(!!) belong to the other cue --> LLM prefers one cue over the other and seems to discard the other cue mostly 
- model is on average slightly more confident in shape responses

Additional paragraph: combination of both leads to ....

# Sec. 6 Steering
=> prev section has shown that the LLM has an influence of the bias - can we use this?
=> How flexible is the representation in each modality? 
=> we cannot steer the inductive bias, but influence the bias in the output by alterations of the input


6.1 Vision Steering
=> How far can we steer the bias in vision?
Experiment: "Perturb" cue-conflict: either add Gaussian noise (increase texture bias), or slice and shuffle (increase texture bias)
Results:
- LLaVA: 8.4 to 89.5\% shape bias (at drop in accuracy), similar results on the encoder (CLIP), tho LLaVA is slightly more shape bias
- InternVL 1.1 6.1 to 91.7\% shape bias => some models seem to be more steerable
Discussion: We need to clearly outline that this "steers" by eliminating one cue. This impacts accuracy even on a simple dataset like cue-conflict (16 classes; > 50\% acc. in all cases)

6.2 Language steering
=> Given the (default) vision representation, how much can the LLM steer?


-- TODO: show accuracies (full table in appendix?)
-- TODO: appendix: plot acc vs shape bias

Experiment: Neutral vs. texture/shape-biased prompts on VQA for some models
Results: 
- Shifts shape bias in the corresponding direction
- More steerable in texture direction, shape increase is rather minor
- Accuracy is largely not affected contrary to vision steering!

Experiment: Do models even understand texture shape/bias? --> test synonyms from thesaurus (LLaVA, InternVL 1.1)
Results: 
- Synonyms cluster relatively nicely --> slightly more variance for texture due to some poor synonyms

Experiment: Does a larger LLM ensure more steerability? --> InternVL 1.2+ vs 1.1
Result: No.

Experiment: Do better prompts exist? Use LLM to search:
Results: Yes, up to 23.3\% range on InternVL 1.1 with LLM prompts. Extremes show some more drop in accuracy. Limitation: optimization on test set...

- Link to psychophysical results: humans can also not be more shape biased, and steerability toward texture is also not able to fundamentally change shape bias

(6.3 Multimodal combination)


# Appendix

-> Do shape-biased prompts help robustness?

